Implementing a Quantum Coin Scheme

Quantum computing has the power to break current cryptographic systems, disrupting online banking, shopping, data storage and communications. Quantum computing also has the power to support stronger more resistant technologies. In this paper, we describe a digital cash scheme created by Dmitry Gavinsky, which utilises the capability of quantum computing. We contribute by setting out the methods for implementing this scheme. For both the creation and verification of quantum coins we convert the algebraic steps into computing steps. As part of this, we describe the methods used to convert information stored on classical bits to information stored on quantum bits.

==> name.tex <==
\section{Creation of $\mathcal{Q}$ coins}
First let us describe Gavinsky's definition of a coin, named $\mathcal{Q}$-coin, then we will describe how it is created.
\begin{defn}[$\mathcal{Q}$-coins]
Let $3|t$. For each coin a secret record exists consisting of $k$ entries $x_1, \dots, x_k$ s.t. $x_i \in \{0,1\}^4$ (i.e., the secret record contains $k$ strings of $4$ classical bits). A ``fresh'' $\mathcal{Q}$-coin is then created corresponding to this record $(x_1,\dots, x_k)$. This coin consists of:
\begin{itemize}
    \item $k$ quantum registers consisting of 2 qubits each, where the $i$'th register contains $\ket{\alpha(x_i)}$;
    \item a $k$-bit classical register P, that is initially set to $0^k$;
    \item a unique identification number.
\end{itemize}
\end{defn}


Creation of the coins requires the conversion of the 4 classical bits to two quantum bits. 

\begin{defn}[$\textit{HMP}_4$-\textit{states}]
    Let $x \in \{0,1\}^4$. The corresponding $\textit{HMP}_4$-\textit{state} is 
    \[
        \ket{\alpha(x)} \myeq \frac{1}{\sqrt{4}} \sum_{1 \leq i \leq 4} (-1)^{x_i} \ket{i}.
    \]
\end{defn}


Algebraically this formula perfectly represents the conversion of 4 bits to 2 qubits. For example, the string of 4 classical bits $[0 1 1 0]^T$ is converted to qubits as 
\begin{align*}
     \ket{\alpha([0 1 1 0]^T)} &= \frac{1}{\sqrt{4}} \huge((-1)^{0} \ket{1} + (-1)^{1} \ket{2} + (-1)^{1} \ket{3} + (-1)^{0} \ket{4}\huge)\\
     &= \frac{1}{2} \huge(\ket{1}  - \ket{2} - \ket{3} +  \ket{4}\huge)
\end{align*}

\subsection{Implementation}\label{sec:create}
 We wish to create  a pair of quantum bits corresponding to each of the 16 possible arrangements of the 4 classical bits. To effect the same conversion computationally we need to manipulate a starting pair of qubits. To create the first 8 quantum representations of the classical strings we take two qubits separately. To convert the remaining 8 classical strings we need to first entangle our starting qubits.  

\subsubsection{No entanglement}
\begin{itemize}
    \item Given any two quantum bits. Let $q_1 = \alpha\ket{0} +\beta\ket{1}$ and $q_2 = \gamma\ket{0} +\delta\ket{1}$.
    \item The state space\footnote{The state space of a composite systems is the tensor product of the state spaces of the component physical systems.} of these two bits is
    \begin{align}
        q_1 \otimes q_2 = (\alpha\ket{0} +\beta\ket{1})(\gamma\ket{0} +\delta\ket{1}) &= \alpha\gamma\ket{00} + \alpha\delta\ket{01} + \beta\gamma\ket{10} + \beta\delta\ket{11}\\ &= \alpha\gamma\ket{1} + \alpha\delta\ket{2}  + \beta\gamma\ket{3} + \beta\gamma\ket{4}\\
        &\equiv \begin{bmatrix} \alpha\gamma & \alpha\delta & \beta\gamma & \beta\gamma\end{bmatrix}^T
    \end{align} 
    \item $\alpha, \beta,\gamma$ and $\delta$ can each take either -1 or +1. Thus we we can create: \\
    \begin{center}
    \begin{tabular}{L L L L}
        \alpha=-1 & \beta,\gamma,\delta=1 & \rightarrow & \begin{bmatrix} -1 & -1 & \hphantom{+}1 & \hphantom{+}1\end{bmatrix}^T  =\ket{Q_1}\\
        \beta=-1 & \alpha,\gamma,\delta=1 & \rightarrow & \begin{bmatrix} \hphantom{+}1 & \hphantom{+}1 & -1 & -1\end{bmatrix}^T =\ket{Q_2}\\
        \gamma=-1 & \alpha,\beta,\delta=1 & \rightarrow & \begin{bmatrix} -1 & \hphantom{+}1 & -1 & \hphantom{+}1\end{bmatrix}^T =\ket{Q_3}\\
        \delta=-1 & \alpha,\beta,\gamma=1 & \rightarrow & \begin{bmatrix} \hphantom{+}1 & -1 & \hphantom{+}1 & -1\end{bmatrix}^T =\ket{Q_4}\\
        \alpha,\beta=-1 & \gamma,\delta=1 & \rightarrow & \begin{bmatrix} -1 & -1 & -1 & -1\end{bmatrix}^T =\ket{Q_5}\\
        \alpha,\gamma=-1 & \beta,\delta=1 & \rightarrow & \begin{bmatrix} \hphantom{+}1 & -1 & -1 & \hphantom{+}1\end{bmatrix}^T =\ket{Q_6}\\
        \alpha,\delta=-1 & \beta,\gamma=1 & \rightarrow & \begin{bmatrix} -1 & \hphantom{+}1 & \hphantom{+}1 & -1\end{bmatrix}^T =\ket{Q_7}\\
        \alpha,\beta,\gamma,\delta=-1 & &\rightarrow & \begin{bmatrix} \hphantom{+}1 & \hphantom{+}1 & \hphantom{+}1 & \hphantom{+}1\end{bmatrix}^T=\ket{Q_8}\\
    \end{tabular}
    \end{center}
    \item All other combinations give repetitions of these 8 quantum states. 
\end{itemize}
\subsubsection{With entanglement}
\begin{itemize}
    \item First let us create entangled qubits. 
    \begin{defn}[Bell States]
   Bell states are four specific maximally entangled quantum states of two qubits. They are in a superposition of 0 and 1. the four states are:
   \begin{align}
       &\ket{\Phi^+}= \frac{1}{\sqrt{2}}(\ket{0}_A \otimes \ket{0}_B + \ket{1}_A \otimes \ket{1}_B) =  \begin{bmatrix} 1&0&0&1\end{bmatrix}^T\\
       & \ket{\Phi^-}= \frac{1}{\sqrt{2}}(\ket{0}_A \otimes \ket{0}_B - \ket{1}_A \otimes \ket{1}_B) = \begin{bmatrix} 1&0&0&-1\end{bmatrix}^T\\
       &\ket{\Psi^+}= \frac{1}{\sqrt{2}}(\ket{0}_A \otimes \ket{1}_B + \ket{1}_A \otimes \ket{0}_B) = \begin{bmatrix} 0&1&1&0\end{bmatrix}^T\\
       &\ket{\Psi^-}= \frac{1}{\sqrt{2}}(\ket{0}_A \otimes \ket{1}_B - \ket{1}_A \otimes \ket{0}_B) = \begin{bmatrix} 1&0&-1&0\end{bmatrix}^T
   \end{align}
    \end{defn}
    \item These Bell states can each be created by taking a computational basis as the input and putting this through a Hadamard gate and a CNOT gate.  As an example, Figure~\ref{fig:diag1} shows a quantum circuit with a Hadamard-CNOT combination. Given input \ket{00} it produces the Bell state \ket{\Phi^+}.
    \input{diagram.tex}
    \item Using the now entangled qubits we can generate the required remaining 8 combinations by putting these through quantum gates. Below we define these gates. 
    \begin{defn}[Hadamard gate]
    The Hadamard gate acts on a single qubit. It maps the basis state \ket{0} to $\frac{\ket{0} + \ket{1}}{\sqrt{2}}$ and \ket{1} to $\frac{\ket{0} - \ket{1}}{\sqrt{2}}$. That is, it creates a superposition where the measurement has equal probability of becoming 0 or 1. It is represented by the Hadamard matrix:
    \[ H = \frac{1}{\sqrt{2}}\begin{bmatrix}1& 1 \\1 &-1 \end{bmatrix}\]
    \end{defn}
    \begin{defn}[Pauli-X gate]
    The Pauli-X gate acts on a single qubit. It is the quantum equivalent of the NOT gate for classical computers. Due to this nature, it is sometimes called bit-flip. It maps \ket{0} to \ket{1} and visa versa. It is represented by the Pauli X matrix: 
    \[ X =\begin{bmatrix}0& 1 \\1 &0 \end{bmatrix}\]
    \end{defn}
    \begin{defn}[Pauli-Z gate]
    The Pauli-Z gate acts on a single qubit. It equates to a rotation around the Z-axis of the Bloch sphere by $\pi$ radians. It leaves the basis state \ket{0} unchanged and maps \ket{1} to -\ket{1}. It is sometimes called phase-flip. It is represented by the Pauli Z matrix:
    \[ Z =\begin{bmatrix}1& 0 \\0 &-1 \end{bmatrix}\]
    \end{defn}
    \begin{defn}
        The swap gate swaps two qubits. It is represented by the matrix: 
        \[ \textit{SWAP} =\begin{bmatrix}1& 0 &0&0\\0&0&1&0\\0&1&0&0\\0&0&0&1 \end{bmatrix}\]
    \end{defn}
    %
    An example of these gates acting on the entangles qubits is shown in Figure~\ref{fig:diag2}. It shows the entangled Bell state \ket{\Phi^+} passed through an extended Hadamard gate.
    \input{diagram2.tex}
    \item Below we depict the combination of gates used to create the 8 linear combinations. $I$ denotes the identity matrix, $\otimes$ denotes the tensor product (gates wired in parallel) and $\times$ denotes the ordinary matrix cross product (serially wired gates).
    \begin{center}
        \begin{tabular}{L L L}
             (H \otimes I) \times \ket{\Phi^+}&  \rightarrow &  \frac{1}{2}\begin{bmatrix} \hphantom{+}1 & \hphantom{+}1 & \hphantom{+}1 & -1\end{bmatrix}^T =\ket{Q_9}\\
             %
             (H \otimes I) \times \ket{\Psi^+}&  \rightarrow &  \frac{1}{2}\begin{bmatrix} \hphantom{+}1 & \hphantom{+}1 & -1 & \hphantom{+}1\end{bmatrix}^T  =\ket{Q_{10}}\\
             %
             (H \otimes I) \times \ket{\Phi^-}&  \rightarrow &  \frac{1}{2}\begin{bmatrix} \hphantom{+}1 & -1 & \hphantom{+}1 & \hphantom{+}1\end{bmatrix}^T =\ket{Q_{11}}\\
             %
             (X \otimes I) \times \ket{Q_{10}} & \rightarrow &  \frac{1}{2}\begin{bmatrix} -1 & \hphantom{+}1 & \hphantom{+}1 & \hphantom{+}1\end{bmatrix}^T =\ket{Q_{12}}\\
             %
             (Z \otimes I) \times \ket{Q_{11}}& \rightarrow & \frac{1}{2}\begin{bmatrix} \hphantom{+}1 & -1 & -1 & -1\end{bmatrix}^T =\ket{Q_{13}}\\
             %
             (Z \otimes I) \times \ket{Q_{12}}& \rightarrow & \frac{1}{2}\begin{bmatrix} -1 & \hphantom{+}1 & -1 & -1\end{bmatrix}^T =\ket{Q_{14}}\\
            %
            (I \otimes Z) \times \ket{Q_{12}}& \rightarrow & \frac{1}{2}\begin{bmatrix} -1 & -1 & \hphantom{+}1 & -1\end{bmatrix}^T =\ket{Q_{15}}\\
            %
            (X \otimes I) \times \ket{Q_{14}}& \rightarrow & \frac{1}{2}\begin{bmatrix} -1 & -1 & -1 & \hphantom{+}1\end{bmatrix}^T =\ket{Q_{16}}\\
             %
             
             %
            
            
             %(I \otimes H) \times \ket{\Psi^-}& \rightarrow & \frac{1}{2}\begin{bmatrix} \hphantom{+}1 & \hphantom{+}1 & -1 & -1\end{bmatrix}^T 
           
        \end{tabular}
    \end{center}
    \item For the creation of quantum coin, this mapping of classical bits to quantum bits can be hard-coded into the system. Therefore, this work only needs to be completed once. 
    \item As described in \cite{garcia2011equivalent} there are alternative circuit configurations which will produce equivalent results.
\end{itemize}
